Iterative compilation on mobile devices

The abundance of poorly optimized mobile applications coupled with their increasing centrality in our digital lives make a framework for mobile app optimization an imperative. While tuning strategies for desktop and server applications have a long history, it is difficult to adapt them for use on mobile phones. Reference inputs which trigger behavior similar to a mobile application's typical are hard to construct. For many classes of applications the very concept of typical behavior is nonexistent, each user interacting with the application in very different ways. In contexts like this, optimization strategies need to evaluate their effectiveness against real user input, but doing so online runs the risk of user dissatisfaction when suboptimal optimizations are evaluated. In this paper we present an iterative compiler which employs a novel capture and replay technique in order to collect real user input and use it later to evaluate different transformations offline. The proposed mechanism identifies and stores only the set of memory pages needed to replay the most heavily used functions of the application. At idle periods, this minimal state is combined with different binaries of the application, each one build with different optimizations enabled. Replaying the targeted functions allows us to evaluate the effectiveness of each set of optimizations for the actual way the user interacts with the application. For the BEEBS benchmark suite, our approach was able to improve performance by up to 57%, while keeping the slowdown experienced by the user on average at 0.8%. By focusing only on heavily used functions, we are able to conserve storage space by between two and three orders of magnitude compared to typical capture and replay implementations.

==> Makefile <==
TEX = hipeac.tex 

CLS = sig-alternate.cls

PACKAGE = hipeac

PDF = ${TEX:%.tex=%.pdf}

PWD= ${shell pwd}

all: $(PDF)

%.pdf: $(CLS) ${shell ls *.tex}
	pdflatex $*
	bibtex hipeac
	pdflatex $*
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log)\
	do pdflatex $*; done
	#gs -sFONTPATH=/usr/share/fonts/truetype/droid:/usr/share/texlive/texmf-dist/fonts/vf/public/droid \
	#	-o powercap2.pdf -sDEVICE=pdfwrite -dPDFSETTINGS=/prepress powercap.pdf
	gs -o temp.pdf -sDEVICE=pdfwrite -dPDFSETTINGS=/prepress $(PDF)
	mv temp.pdf $(PDF)

clean:
	$(RM) *.aux *.log  *.blg hipeac.pdf

distclean: clean
	$(RM) $(PDF) *.bbl

zip: all clean
	zip $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> futureWork.tex <==
%%%%%%%%%%%%%%%%%%
%  FUTURE WORK (I put this in a last paragraph on Conclusion)
%%%%%%%%%%%%%%%%%%

%\section{Future work}\label{sec:futureWork}
% reduce the overhead even more
% make it on Android apps + real interactive apps.
% challenges in this new territory

%Why is engineering work:
%In our future work, we plan to integrate our iter optimiser with the android application compiler which is dex2oat.
%The dex2oat compile the java bytecode found in android application packages, into native code.
%A flavor of dex2oat, called optimising, provides some optimisation options, but still they are far less options than other compiler infrastructures like llvm, and it is still under heavy development.
%the main focus of its developers was the speed because many of the compilations happen while users use their devices, for example when they install new apps, update existing ones, or perform an OS update to their device.
%There was an llvm flavor as well, but the support was dropped a while ago because of the speed of the compiler.
%Since we do not have problem regarding the compilation time, an infrastructure with more options would be preferable.
%Additionally, only a small fraction of the code is going to be recompiled.
%So a real life system could have used android's low overhead profiling techniques to extract the hot functions, and then
%use an android compiler to apply iterative optimisation on them.
%Since we consider such integration more engineer work than contribution to science we have decided not to implement it, at least until
%the optimising version of the compiler becomes stable enough. 
%We plan to proceed to this implementation though, because in our future plans is  to further exploit the captured data by 
%using extra information that is available in Java bytecode and not in C programs.
